On weakly amenable groupoids

In this work, we study groupoids and their approximation properties, generalizing both the definitions and some known results for the group case. More precisely, we introduce weak amenability for groupoids using the definition of the Fourier algebra given by Renault. We prove that weakly amenable groupoids are inner exact. We also generalize its algebraic counterpart, the CBAP. To do this we introduce the notion of a quasi Cartan pair $(B,A)$ and see that $(C_r^*(G),C_0(G^0))$ can be viewed as such. We then define what it means for a pair $(B,A)$ to have the CBAP. We introduce the Cowling-Haagerup constants associated to these approximation properties and prove that $\Lambda_{\text{cb}}(C_r^*(G),C_0(G^0)) \leq \Lambda_{\text{cb}}(G)$. We then study some classes of groupoids where we could achieve equality, that is, $\Lambda_{\text{cb}}(G) = \Lambda_{\text{cb}}(C_r^*(G),C_0(G^0))$. They are discrete groupoids and groupoids arising from partial actions of a discrete group $\Gamma$ on a locally compact Hausdorff space $X$.

==> Fell_General/Fell_Absorption.tex <==
\section{Fell Absorption}
Given a covariant representation $(\pi,v)$ of $(A,\beta,S)$ on $H$, define the spaces $H_s := \pi(A_s)H$. We now want to induce a new covariant representation on $\ell^2(S) \otimes H$ by setting for $a \in A$, $t \in S$ and $\xi \in H$,
$$
\Ind_\pi(a)(\delta_t \otimes \xi) = \begin{cases}
    \delta_t \otimes \pi(a)\xi \quad &\text{ if } a \in A_t,\xi \in H_t, \\
    0 &\text{ otherwise.}
\end{cases}
$$
and for $s \in S$
$$
(\lambda^S \otimes v)(s)(\delta_t \otimes \xi ) = \lambda_{s}^S\delta_t \otimes v_s\xi = \begin{cases}
    \delta_{st} \otimes v_s\xi \quad &\text{ if } r(t) \leq d(s), \\
    0 &\text{ otherwise.}
\end{cases}
$$
\begin{prop}
    The pair $(\Ind_\pi,\lambda^S \otimes v)$ is a covariant representation of $(A,\beta,S)$.
\end{prop}
\begin{proof}
Let $s,t \in S$, $a \in A_{s^*} = C(r(s))$ and $\xi \in H$, we start by proving that 
$$
\left( \lambda^S_s \otimes v_s \right) \Ind_\pi(a) \left( \lambda^S_{s^*} \otimes v_{s^*} \right)(\delta_t \otimes \xi) = \Ind_\pi(\beta_s(a))(\delta_t \otimes \xi)
$$
We compute the left side to be (recall that $\supp(a) \subseteq r(s)$)
    \begin{align*}
      &\begin{cases}
    \left( \lambda^S_s \otimes v_s \right) \Ind_\pi(a)(\delta_{s^*t} \otimes v_{s^*}\xi) \quad &\text{ if } r(t) \leq r(s), \\
    0 &\text{ otherwise.} 
    \end{cases}\\
    =& \begin{cases}
     \left( \lambda^S_s \otimes v_s \right)(\delta_{s^*t} \otimes \pi(a)v_{s^*}\xi) \quad &\text{ if } r(t) \subseteq \supp(a) \text{ and } r(t) \leq r(s), \\
    0 &\text{ otherwise.}
    \end{cases} \\
    =& \begin{cases}
     \delta_{ss^*t} \otimes v_s\pi(a)v_{s^*}\xi \quad &\text{ if } r(t) \subseteq \supp(a) \cap r(s), \\
    0 &\text{ otherwise.}
    \end{cases} \\
    =& \begin{cases}
     \delta_{t} \otimes \pi(\beta_s(a))\xi \quad &\text{ if } r(t) \subseteq \supp(a), \\
    0 &\text{ otherwise.}
    \end{cases} 
\end{align*}
which is equal to $\Ind_\pi(\beta_s(s))(\delta_t \otimes \xi)$. For $e \in E$, we observe that
\begin{align*}
   \im \! \! \left( \lambda^S_e \otimes v_e \right) = \cls \{\delta_u \otimes \eta: r(u) \leq e, \eta \in \im(v_e) = \pi(A_e)H \}.
\end{align*}
On the other hand, for $e \in E$,
\begin{align*}
    \Ind_\pi(a)(\delta_t \otimes \xi) = \begin{cases}
    \delta_t \otimes \pi(a)\xi \quad &\text{ if } r(t) \subseteq \supp(a) \subseteq e, \\
    0 &\text{ otherwise.}
    \end{cases}
    \in \im \! \! \left( \lambda^S_e \otimes v_e \right),
\end{align*}
for all $a \in A_e = C(e),t \in S, \xi \in H$. Conversely, if $\delta_u \otimes \eta \in \im \! \! \left( \lambda^S_e \otimes v_e \right)$, by picking $a = \chi_e$ we get that 
$$
\Ind_\pi(1_s)(\delta_u \otimes \eta) = \delta_u \otimes \eta.
$$
We conclude 
$$
\im \! \! \left( \lambda^S_e \otimes v_e \right) = \Ind_\pi(A_e)(\ell^2(S) \otimes H).  
$$
\end{proof}
\begin{theorem}
Let $(\pi,v)$ be a covariant representation of $(C(X),\beta,S)$ on $H$ with induced covariant representation $(\Ind_\pi,\lambda^S \otimes v)$. Moreover, let $(\iota, \lambda^\beta)$ be the left regular covariant representation. Then there exists a partial isometry $W: \ell^2_\beta(S,A) \otimes H \xrightarrow{} \ell^2(S) \otimes H$ intertwining $(\Ind_\pi,\lambda^S \otimes v)$ with $(\iota \otimes 1,\lambda^\beta \otimes 1)$, that is, such that 
$$
\lambda^S \otimes v = W\left( \lambda^\beta \otimes 1 \right)W^* \quad \text{ and } \quad \Ind_\pi = W(\iota \otimes 1)W^*.
$$
\end{theorem}
\begin{proof}
    Define 
    $$
W(a\delta_t \otimes \xi) = \delta_t \otimes \pi(a)v_t\xi
    $$
    Compute for $s \in S$
    \begin{align*}
W\left( \lambda^\beta_s \otimes 1 \right)(b\delta_t \otimes \xi) = W(b\delta_{st} \otimes \xi) = \delta_{st} \otimes \pi(b)v_{st}\xi,
    \end{align*}
for all $b\delta_t \otimes \xi$. On the other hand
    \begin{align*}
        \left(\lambda^S_s \otimes v_s\right) W (b\delta_t \otimes \xi) = \left(\lambda^S_s \otimes v_s\right)(\delta_t \otimes \pi(b)v_t\xi) = \begin{cases}
            \delta_{st} \otimes v_s\pi(b)v_t\xi &\text{ if } r(t) \leq d(s), \\
            0 &\text{ otherwise.}
        \end{cases}
    \end{align*}
\end{proof}


==> Fell_General/Inverse_Semigroup_Actions.tex <==
\section{Inverse Semigroup Actions on $C^*$-algebras}
Let $X$ be a locally compact Hausdorff Space we denote by $\mathcal{I}(X)$ the set of all partial homeomorphisms of $X$, it is an inverse semigroup under the operation given by composition. In this section, we discuss actions of an inverse semigroup $S$ on a topological space $X$ and construct a groupoid associated to it. Following that we give the definition of an action of $S$ on a $C^*$-algebra $A$ and build the crossed product $A \rtimes S$.
\begin{defi}\label{actioninv}
An action of $S$ on $X$ is an inverse semigroup homomorphism $\alpha: S \rightarrow \mathcal{I}(X)$ such that
\begin{enumerate}[i]
    \item For every $s \in S$, $\alpha_s$ is continuous and has open domain on $X$;
    \item The union of the domains of all the $\theta_s$'s is $X$.
\end{enumerate}
\end{defi}
For each $s \in S$, we denote the domain of $\alpha_s$ by $D_s = D_{ss^*}$ and we define the subset of $X \times S$ 
$$
\Xi := \{(x,s) \in X \times S: x \in D_s \},
$$
on it we define an equivalence relation $(x,s) \sim (y,t)$ if and only if $x = y$ and there exists $e \in E$ such that $x \in D_e$ and $se = te$. For $(x,s) \in \Xi$ we denote its equivalence class by $[x,s]$ which is called the \textit{germ of $s$ at $x$}. We let $X \rtimes_\alpha S := \Xi / \sim$ (or just $X \rtimes S$ when $\alpha$ is obvious from the context) and define range and source maps as $d([x,s]) = [x,ss^*],r([x,s]) = [\alpha_s(x),ss^*]$, moreover we define a product by
$$
[\alpha_t(x),s][x,t] = [x,st]
$$
and inverse $[x,s]^{-1} = [\alpha_s(x),s^*]$. It remains to topologize $X \rtimes S$, for each $s \in S$ and open $U \subseteq D_s$, let 
$$
D(U,s) = \{ [x,s] \in X \rtimes S: x \in U \}
$$
\begin{prop}[{\cite[Proposition 4.17]{exel2008inverse}}]\label{gofgerms}
    The sets $D(U,s)$ are a basis for a topology on $X \rtimes_\alpha S$. Moreover, the operations defined above turn $X \rtimes_\alpha S$ into an étale groupoid.
\end{prop}
The groupoid $X \rtimes_\alpha S$ will be called the \textit{groupoid of germs of the action $(X,\alpha,S)$}.
\begin{example}\label{canact}
    Suppose $\G$ is any étale groupoid, recall the canonical action of $\G^{op}$ on $X = \gob$ given by
    $$
\alpha_U(x) = UxU^{-1}, \quad \text{ for all } x \in d(U),
$$
it is indeed an action in the sense of Definition \ref{actioninv}, with domain $d(U)$ and range $r(U)$. Moreover, if $S \subseteq \G^{op}$ is an inverse subsemigroup then one can restrict $\alpha$ to $S$ and the following proposition shows under what conditions we have $X \rtimes_{\alpha|_S} S \cong \G$.
\end{example}
\begin{prop}[{\cite[Proposition 5.4]{exel2008inverse}}]\label{isotrans}
Let $\G$ be an étale groupoid and $S \subseteq \G^{op}$ be an inverse subsemigroup such that 
\begin{enumerate}[(i)]
    \item $\bigcup\limits_{U \in S} U = \G$, and 
    \item for every $U,V \in S$ and $u \in U \cap V$, there exists $W \in S$ such that $u \in W \subseteq U \cap V$.
\end{enumerate}
Then we have that $X \rtimes_{\alpha|_S} S \cong \G$.
\end{prop}
We now turn our attention to actions of inverse semigroups on a $C^*$-algebra $A$.
\begin{defi}
    A \textit{partial automorphism} of $A$ is a triple $(\alpha,I,J)$ where $I,J \subseteq A$ are closed ideals and $\alpha:I \rightarrow J$ is a $*$-isomorphism. 
\end{defi}
We denote the set of partial automorphisms of $A$ by $\PAut(A)$ and it is easy to see that it is an inverse semigroup.
\begin{defi}\label{actioninvalg}
    Let $S$ be an inverse semigroup and $A$ a $C^*$-algebra. An \textit{action of $S$ on $A$} is a homomorphism $\beta: S\rightarrow \PAut(A)$ such that:
    \begin{enumerate}[(i)]
        \item $s \mapsto \beta_s = (\alpha_s,A_{s^*},A_s)$ is a partial automorphism;
        \item the set $\bigcup_{s \in S} A_s$ is a dense subalgebra of $A$.
    \end{enumerate}
\end{defi}
\begin{defi}
    Let $\beta$ be an action of $S$ on $A$, a \textit{covariant representation of $(A,\beta,S)$} is a triple $(\pi,v,H)$ where $\pi:A \rightarrow B(H),v: S \rightarrow B(H)$ are nondegenerate $*$-representations such that for all $a \in A,s \in S$
    \begin{enumerate}[(i)]
        \item $v_s\pi(a)v_{s^*} = \pi(\beta_s(a))$, for all $a \in A_{s^*}$;
        \item $v_s$ has initial subspace $\pi(A_{s^*})H$ and final subspace $\pi(A_{s})H$.
    \end{enumerate}
\end{defi}
In order to construct the crossed product, we consider the space $C_c(S,A)$ and introduce the subspace 
$$
C_c^\beta(S,A) := \{ f \in C_c(S,A): f(s) \in A_s, \text{ for all } s \in S\}.
$$
Moreover, we define a multiplication and involution on $C_c^\beta(S,A)$ as follows: for $a,b \in A$ and $s,t \in S$
$$
(a\delta_s)(b\delta_t) = \beta_{s}(\beta_{s^*}(a)b)\delta_{st} \, ; \quad (a\delta_s)^* = \beta_{s^*}(a^*)\delta_{s^*},
$$ 
this way, $C_c^\beta(S,A)$ becomes a $*$-algebra. If $f,g \in C_c^\beta(S,A)$ are arbitrary functions, we will denote their product by $f*g$. Now, given a covariant  $(\pi,v,H)$ representation of $(A,\beta,S)$ we can induce a representation $\pi \rtimes v$ of $C_c^\beta(S,A)$ defined for $a \in A, s \in S$ by
$$
\pi \rtimes v (a\delta_s) = \pi(a)v_s.
$$
We are now ready to define a universal seminorm on $C_c^\beta(S,A)$
$$
\|f\|_* := \sup \{ \| \pi \rtimes v(f)\| : (\pi,v,H) \text{ is a covariant representation of } (A,\beta,S) \}.
$$
Letting the ideal $J_S := \{ f \in C_c^\beta(S,A) : \|f\|_* = 0 \}$, the \textit{crossed product of $(A,\beta,S)$} is defined to be the completion of $C_c^\beta(S,A) / J_S$ with respect to $\| \cdot \|_*$ and is denoted by $A \rtimes_\beta S$. The ideal $I$ is rarely trivial, indeed, it can be checked that for all $e_1,e_2 \in E$ and $a \in A_{e_1} \cap A_{e_2}$ then $a\delta_{e_1} - a\delta_{e_2} \in J_S$. With this in mind, we arrive at the following definition.
\begin{defi}
    A nondegenerate $*$-representation $\Pi: C_c^\beta(S,A) \rightarrow B(H)$ is said to be \textit{admissible} if for all $e_1,e_2 \in E$ with $e_1 \leq e_2$ and every $a \in A_{e_1}$ we have that $\Pi(a\delta_{e_1}) = \Pi(a\delta_{e_2})$.
\end{defi}
As expected, we can relate admissible representations of $C_c^\beta(S,A)$ with covariant representations of $(A,\beta,S)$.
\begin{theorem}[{\cite[Lemma 9.6 and Proposition 9.7]{exel2008inverse}}]\label{covariant reps theorem}
Let $\Pi: C_c^\beta(S,A) \rightarrow B(H)$ be an admissible nondegenerate $*$-representation, define 
$\pi: A \rightarrow B(H)$ by 
$$
\pi(a) = \Pi(a\delta_e), \quad \text{ for all } e \in E, a \in A_e.
$$
Define also $v: S \rightarrow B(H)$ by 
$$
v_s = \text{s-}\!\lim\limits_\lambda \Pi(u_\lambda \delta_s),
$$
where $\{u_\lambda\}$ is a positive bounded approximate identity for $E_s$. Then $(\pi,v,H)$ is a covariant representation of $(A,\beta,S)$ such that $\Pi = \pi \rtimes v$. Moreover, $(\Pi,H) \mapsto (\pi,v,H)$ is a one-to-one correspondence between admissible non degenerate $*$-representations of $C_c^\beta(S,A)$ and covariant representations of $(A,\beta,S)$.
\end{theorem}
We obtain as a corollary a different way to view the full $C^*$-algebra of a measured étale groupoid $C^*(\G)$.
\begin{corollary}[{\cite[Proposition 9.9]{exel2008inverse}}]
    Let $\G$ be a measured étale groupoid and $S$ be an inverse semigroup satisfying the conditions of Proposition \ref{isotrans}, then $C^*(\G)$ is canonically isomorphic to $C_0(X) \rtimes_\beta S$.
\end{corollary}


==> Fell_General/Left_Regular_Representation.tex <==
\section{Left Regular Representation}
Let $\G$ be a measured Hausdorff ample groupoid such that $X := \gob$ is compact, then $\G^a$ acts on $X$ as in Example \ref{canact}, moreover, let $S \subseteq \G^a$ be any unital subsemigroup satisfying the conditions of Proposition \ref{isotrans}.  The action $\alpha$ induces an action $\beta$ of $S$ on $A := C(X)$ given by 
$$
\beta_s(f)(x) = f(\alpha_{s^*}(x)) \quad \text{ for all } f \in C(d(s)) \text{ and }x \in r(s),
$$ 
Letting $A_s := C(r(s))$, we now turn our attention to the space 
$$
C_c^\beta(S,A) := \{ f \in C_c(S,A): f(s) \in A_s, \text{ for all } s \in S \}
$$
The map $\Delta : C_c^\beta(S,A) \rightarrow C_c(\G)$ given by 
$$
\Delta(a\delta_s)(\gamma) = \begin{cases}
a(r(\gamma)) \quad &\text{ if } \gamma \in s, \\
0 &\text{ otherwise.} 
\end{cases}
$$
implements the isomorphism $A \rtimes_\alpha S \cong C^*(\G)$ of \cite[Proposition 9.9]{exel2008inverse} meaning that it is an isometry between the seminorm $\|\cdot \|_*$ of the previous section and the universal norm on $C_c(\G)$, thus $\ker \Delta = J_S$. An algebraic description of $J_S$ is available to us.
\begin{prop}[{\cite[p.11]{buss2023approximation}}]
The kernel $\ker(\Delta) = J_S$ is equal to the ideal generated by the set
$$
\{ a\delta_s - a\delta_t \in C_c^\beta(S,A): a \in C_0(r(s \cap t)) \}.
$$
\end{prop}
Since in the sequel we will deal with a lot of basis elements, that is, elements of the from $a \delta_s$ with $s \in S$ and $a \in A_s$, the reader might be concerned that they are zero after we quotient, however that is not the case.
\begin{prop}[{\cite[Lemma 2.28]{buss2023approximation}}]
    Let $s \in S$ and $a \in A_s$, then $a\delta_s \notin J_S$.
\end{prop}
From now on we denote $C_c^\beta(S,A,J_S) := C_c^\beta(S,A)/J_S$ and we abuse notation and still denote by $\Delta$ the isomorphism induced by it. Consider the restriction map $E: C_c(\G) \rightarrow A$, since $\G$ is Hausdorff it is a \textit{weak conditional expectation} in the sense of \cite[p. 11]{buss2023approximation}, meaning for all $f \in C_c(\G)$:
\begin{enumerate}[(i)]
    \item $E(f^* * f) \geq 0$,
    \item $E(f^*) = E(f)^*$,
    \item If $f \in C_c(\G) \cap A$, then $E(f) = f$.
\end{enumerate}
Furthermore, $E$ is faithful in the sense that $E(f^* * f) = 0$ implies that $f = 0$. We define for $f,g \in C_c^\beta(S,A,J_S)$ an inner product
$$
\langle f,g \rangle_A =  \int_X E(\Delta(f)^* * \Delta(g)) \, d\mu 
$$
which by completion we obtain the Hilbert space $\ell^2_\beta(S,A)$. 
\begin{prop}
    The map $\Lambda : C_c^\beta(S,A,J_S) \rightarrow B(\ell^2_\beta(S,A))$ given by 
    $$
\Lambda(f)g = f * g, \quad \text{ for all } f \in C_c^\beta(S,A,J_S) \text{ and } g \in \ell^2_\beta(S,A)
    $$
    is a well defined nondegenerate $*$-representation of $C_c^\beta(S,A,J_S)$.
\end{prop}
\begin{defi}
    $\Lambda$ is called the \textit{left regular representation} of the covariant system $(A,\beta,S)$. Moreover, the \textit{reduced crossed product of $A$ by $S$} denoted $A \rtimes_{\beta,r} S $ is defined to be be the closure of $\Lambda(C_c^\beta(S,A,J_S))$ on $B(\ell^2_\beta(S,A))$.
\end{defi}
Recall that for $f,g \in C_c(\G)$ 
$$
\langle f,g \rangle_{L^2(\G,\nu^{-1})} = \int_X E(f^* * g) \, d\mu = \langle \Delta^{-1}(f),\Delta^{-1}(g) \rangle_A.
$$
We have that $\Delta$ extends to a unitary $\ell^2_\beta(S,A) \cong L^2(\G,\nu^{-1})$ which obviously intertwines $\Lambda$ with $\lambda:C_c(\G) \rightarrow B(L^2(\G,\nu^{-1}))$, thus $\Delta$ also extends to an isomorphism $A \rtimes_{\beta,r} S \cong C_r^*(\G) $. \\
\\
Now, we will see what the covariant representation of $(A,\beta,S)$ induced by $\Lambda$ looks like. For this, we use Theorem \ref{covariant reps theorem} and start by letting $\iota: A \rightarrow B(\ell^2_\beta(S,H))$ given by 
$$
\iota(a)(b\delta_t) := \Lambda(a\delta_e)(b\delta_t) = (ab)\delta_{et} = (ab)\delta_t, \quad \text{ for all $e \in E$, $a \in A_e$, $t \in S$ and $b \in A_t$,}
$$
because $ab \in C(r(e \cap t))$. Now, if $s \in S$ and $1_s = \chi_{r(s)} \in A_s$ is the constant one function on $d(s)$, we define
$$
\lambda^{\beta}_s(b\delta_t) := \Lambda(1_s\delta_s)(b\delta_t) =  (1_s\delta_s)(b\delta_t) = \beta_s(\beta_{s^*}(1_s)b)\delta_{st} = \beta_s(1_{s^*} b)\delta_{st}.
$$
Theorem \ref{covariant reps theorem} implies that the pair $(\iota,\lambda^\beta)$ is a covariant representation of $(A,\beta,S)$ such that $\Lambda = \iota \rtimes \lambda^\beta$.
\begin{defi}
    $(\iota,\lambda^\beta)$ will be called the \textit{left regular covariant representation} of $(A,\beta,S)$.
\end{defi}

==> Measurable_Hilbert_Bundles.tex <==
\section{Measurable Hilbert Bundles}

\begin{defi}
    A \textit{measurable Hilbert bundle} is a triple $\hil = (X, \{\hil_x\},\mu)$, where $X$ is a second countable locally compact Hausdorff space, $\{\hil_x\}$ is a collection of Hilbert spaces and $\mu$ is a Borel probability measure on $X$ such that there exists a sequence $e_n: X \rightarrow \cup_{x \in X} \hil_x$ such that:
    \begin{enumerate}[(i)]
        \item For every $n \in \nat$ and $x \in X$, $f(x) \in \hil_x$, that is, each $e_n$ is a section;
        \item For every $n,m \in \nat$, the function $x \mapsto \langle e_n(x),e_m(x) \rangle_{\hil_x}$ is $\mu$-measurable;
        \item For every $x \in X$, the set $\{e_n(x): n \in \nat \}$ span a dense subset of $\hil_x$.
    \end{enumerate}
    Such a sequence $e_n$ is said to be \textit{fundamental}.
\end{defi}
\begin{remark}
    By a Gram-Schmidt process, we can choose $e_n$ to be orthonormal in the sense that for each $x \in X$, the set $\{e_n(x): n \in \nat \}$ is an orthonormal basis of $\hil_x$ \cite[p.91]{paterson2012groupoids}.
\end{remark}
Let us abuse notation and denote also the total space of the bundle by $\hil := \cup_{x \in X} \hil_x$. A section $f: X \rightarrow \hil$ is said to be \textit{measurable} if for all $n \in \nat$, the function $x \mapsto \langle f(x),e_n(x) \rangle_{\hil_x}$ is $\mu$-measurable. The Hilbert space $L^2(X,\hil)$ is defined to be the set of such measurable sections such that $x \mapsto \|f(x)\|^2_{\hil_x}$ is $\mu$-integrable. We thus get an inner product on $L^2(X,\hil)$ defined by 
$$
\langle f,g \rangle := \int_X \langle f(x),g(x) \rangle_{\hil_x} \, d\mu(x),
$$
which indeed turns it to a Hilbert space \cite[p.91]{paterson2012groupoids}.
\begin{defi}
    A section $f: X \rightarrow \hil$ is said to be continuous if for all $n \in \nat$, the function $ x \mapsto \langle f(x),e_n(x) \rangle_{\hil_x} $ is continuous.
\end{defi} 


==> Random/Alcides.tex <==
Seja $S$ um semigrupo inverso e $\G$ o seu grupóide universal. Seja também $\G_S$ o grupóide discreto 
cujo os elementos são os mesmos que de $S$ e o produto está definido para $(s,t) \in S \times S$ que verificam $s^*s = tt^*$, ou seja,
$$
\G_S^{(2)} := \{ (s,t) \in S \times S: s^*s = tt^* \}.
$$
Ao nível dos grupóides acho que consigo obter o mapa 
\begin{align*}
    C_r^*(\G) &\rightarrow C_r^*(\G) \otimes C_r^*(\G_S) \\
     \chi_s   &\mapsto \chi_s \otimes \delta_s
\end{align*}
Em que $\chi_s$ é a função característica em $s \subseteq \G$.

==> Random/Fell_Absorption_for_Inverse_Semigroups.tex <==
\section{Fell Absorption Principle for Inverse Semigroups}
Let $S$ be an inverse semigroup, recall that its left regular representation $\lambda: S \rightarrow B(\ell^2(S))$ is defined for every $s \in S$ as the operator
$$
\lambda_s\delta_t := \begin{cases}
    \delta_{st} \quad &\text{ if } tt^* \leq s^*s, \\
    0 &\text{ otherwise.}
\end{cases}
$$
In this section we prove that the left regular representation $\lambda$ is partially self absorbing in a suitable sense. Let $\pi$ be a representation of $S$ on $H$ and consider the operator
\begin{align*}
    W_\pi: \ell^2(S) \otimes H &\rightarrow \ell^2(S) \otimes H \\
    \delta_s \otimes \xi &\mapsto \delta_s \otimes \pi_s\xi
\end{align*}
it is easy to see that $W^*_\pi(\delta_s \otimes \xi) = \delta_s \otimes \pi_{s^*}\xi$, for all $s \in S,\xi \in H$. We prove that $W_\pi$ is a partial isometry by showing that $W_\pi W^*_\pi W_\pi = W_\pi$. Let $s \in S,\xi \in H$, we compute
\begin{align*}
     W_\pi W^*_\pi W_\pi(\delta_s \otimes \xi) = \delta_s \otimes \pi_{ss^*s}\xi
= \delta_s \otimes \pi_s\xi = W_\pi(\delta_s \otimes \xi),
\end{align*}
thus $W$ is indeed a partial isometry and we denote $\Init(W_\pi), \Fin(W_\pi) \subseteq \ell^2(S) \otimes H$ its initial and final subspace, respectively. We easily compute them to be 
\begin{align*}
    \Init(W_\pi) &= \cls \{ \delta_t \otimes \xi: t \in S \text{ and } \xi \in \Init(\pi_t) \}, \\
    \Fin(W_\pi) &= \cls \{ \delta_t \otimes \xi: t \in S \text{ and } \xi \in \Fin(\pi_t) \}.
\end{align*}
\begin{prop}[Fell's Absorption Principle for Inverse Semigroups]
Let $\pi: S \rightarrow B(H)$ be a representation of $S$ and $\lambda: S \rightarrow B(\ell^2(S))$ the left regular representation, then there exists a partial isometry such that for all $s \in S$,
$$
W_\pi(\lambda_s \otimes 1) = (\lambda_s \otimes \pi_s)W_\pi
$$
\end{prop}
\begin{proof}
    We prove that $W_\pi$ defined above is our desired partial isometry. Let $t \in S,\xi \in H$, we compute
    \begin{align*}
        W_\pi(\lambda_s \otimes 1)(\delta_t \otimes \xi)
        &=
        \begin{cases}
            W_\pi(\delta_{st} \otimes \xi) \quad &\text{ if } tt^* \leq s^*s, \\
            0 &\text{ otherwise.}
        \end{cases}
        = 
        \begin{cases}
            \delta_{st} \otimes \pi_{st}\xi \quad &\text{ if } tt^* \leq s^*s, \\
            0 &\text{ otherwise.}
        \end{cases}
    \end{align*}
    On the other hand,
    \begin{align*}
        (\lambda_s \otimes \pi_s)W_\pi(\delta_t \otimes \xi) =  (\lambda_s \otimes \pi_s)(\delta_t \otimes \pi_t\xi) =
        \begin{cases}
           \delta_{st} \otimes \pi_{st}\xi \quad &\text{ if } tt^* \leq s^*s, \\
            0 &\text{ otherwise.}
        \end{cases}
    \end{align*}  
\end{proof}
\begin{lema}\label{embtensor}
    Let $H,K$ be Hilbert spaces and $\{e_n\}$ an orthonormal basis for $K$. Let $W:H \otimes K \rightarrow H \otimes K$ be a partial isometry. Assume that for all $n \in \nat$, there exist a non-zero $\xi \in H$ such that $e_n \otimes \xi \in \Init(W)$. Let $A \subseteq B(H)$ such that for all $T \in A$, $(T \otimes 1)(\Init(W)) \subseteq \Init(W)$, then the map 
    $$
  \pi:  A \ni T \mapsto W(T \otimes 1)W^* \in B(H)
    $$
    is injective.
\end{lema}
\begin{proof}
    Assume $W(T \otimes 1)W^*=0$, let $n \in \nat$ and $\xi \neq 0$ such that $e_n \otimes \xi \in \Init(W)$ so that $W(e_n \otimes \xi) \in \Fin(W)$, then 
    $$
W(T \otimes 1)W^*(W(e_n \otimes \xi)) = W(T \otimes 1)(e_n \otimes \xi) = W(Te_n \otimes \xi) = 0.
    $$
    Since $T \otimes 1$ is invariant for $\Init(W)$ in which $W$ is isometric we conclude 
    $Te_n \otimes v = 0$. Recalling that $\xi \neq 0$ we get $Te_n = 0$ and since $n$ is arbitrary, $T=0$ as desired.
\end{proof}





==> Random/Ind.tex <==
\section{Fell Absorption}
Given a covariant representation $(\pi,v)$ of $(A,\beta,S)$ on $H$, define the spaces $H_s := \pi(A_s)H$. We now want to induce a new covariant representation on $\ell^2(S) \otimes H$ by setting for $a \in A$, $t \in S$ and $\xi \in H$,
$$
\Ind_\pi(a)(\delta_t \otimes \xi) = \begin{cases}
    \delta_t \otimes \pi(a)\xi \quad &\text{ if } r(t) \subseteq \supp(a), \\
    0 &\text{ otherwise.}
\end{cases}
$$
and for $s \in S$
$$
(\lambda^S \otimes v)(s)(\delta_t \otimes \xi ) = \lambda_{s}^S\delta_t \otimes v_s\xi = \begin{cases}
    \delta_{st} \otimes v_s\xi \quad &\text{ if } r(t) \leq d(s), \\
    0 &\text{ otherwise.}
\end{cases}
$$
\begin{prop}
    The pair $(\Ind_\pi,\lambda^S \otimes v)$ is a covariant representation of $(A,\beta,S)$.
\end{prop}
\begin{proof}
Let $s,t \in S$, $a \in A_{s^*} = C(r(s))$ and $\xi \in H$, we start by proving that 
$$
\left( \lambda^S_s \otimes v_s \right) \Ind_\pi(a) \left( \lambda^S_{s^*} \otimes v_{s^*} \right)(\delta_t \otimes \xi) = \Ind_\pi(\beta_s(a))(\delta_t \otimes \xi)
$$
We compute the left side to be (recall that $\supp(a) \subseteq r(s)$)
    \begin{align*}
      &\begin{cases}
    \left( \lambda^S_s \otimes v_s \right) \Ind_\pi(a)(\delta_{s^*t} \otimes v_{s^*}\xi) \quad &\text{ if } r(t) \leq r(s), \\
    0 &\text{ otherwise.} 
    \end{cases}\\
    =& \begin{cases}
     \left( \lambda^S_s \otimes v_s \right)(\delta_{s^*t} \otimes \pi(a)v_{s^*}\xi) \quad &\text{ if } r(t) \subseteq \supp(a) \text{ and } r(t) \leq r(s), \\
    0 &\text{ otherwise.}
    \end{cases} \\
    =& \begin{cases}
     \delta_{ss^*t} \otimes v_s\pi(a)v_{s^*}\xi \quad &\text{ if } r(t) \subseteq \supp(a) \cap r(s), \\
    0 &\text{ otherwise.}
    \end{cases} \\
    =& \begin{cases}
     \delta_{t} \otimes \pi(\beta_s(a))\xi \quad &\text{ if } r(t) \subseteq \supp(a), \\
    0 &\text{ otherwise.}
    \end{cases} 
\end{align*}
which is equal to $\Ind_\pi(\beta_s(s))(\delta_t \otimes \xi)$. For $e \in E$, we observe that
\begin{align*}
   \im \! \! \left( \lambda^S_e \otimes v_e \right) = \cls \{\delta_u \otimes \eta: r(u) \leq e, \eta \in \im(v_e) = \pi(A_e)H \}.
\end{align*}
On the other hand, for $e \in E$,
\begin{align*}
    \Ind_\pi(a)(\delta_t \otimes \xi) = \begin{cases}
    \delta_t \otimes \pi(a)\xi \quad &\text{ if } r(t) \subseteq \supp(a) \subseteq e, \\
    0 &\text{ otherwise.}
    \end{cases}
    \in \im \! \! \left( \lambda^S_e \otimes v_e \right),
\end{align*}
for all $a \in A_e = C(e),t \in S, \xi \in H$. Conversely, if $\delta_u \otimes \eta \in \im \! \! \left( \lambda^S_e \otimes v_e \right)$, by picking $a = \chi_e$ we get that 
$$
\Ind_\pi(1_s)(\delta_u \otimes \eta) = \delta_u \otimes \eta.
$$
We conclude 
$$
\im \! \! \left( \lambda^S_e \otimes v_e \right) = \Ind_\pi(A_e)(\ell^2(S) \otimes H).  
$$
\end{proof}
\begin{theorem}
Let $(\pi,v)$ be a covariant representation of $(C(X),\beta,S)$ on $H$ with induced covariant representation $(\Ind_\pi,\lambda^S \otimes v)$. Moreover, let $(\iota, \lambda^\beta)$ be the left regular covariant representation. Then there exists a partial isometry $W: \ell^2_\beta(S,A) \otimes H \xrightarrow{} \ell^2(S) \otimes H$ intertwining $(\Ind_\pi,\lambda^S \otimes v)$ with $(\iota \otimes 1,\lambda^\beta \otimes 1)$, that is, such that 
$$
\lambda^S \otimes v = W\left( \lambda^\beta \otimes 1 \right)W^* \quad \text{ and } \quad \Ind_\pi = W(\iota \otimes 1)W^*.
$$
\end{theorem}
\begin{proof}
    Define 
    $$
W(a\delta_s \otimes \xi) = \delta_s \otimes \pi(a)v_s\xi
    $$
    Compute for $s \in S$ and $a \in C(d(s))$
    \begin{align*}
W\left( \lambda^\beta(a\delta_s) \otimes 1 \right)W^*(\delta_t \otimes \xi) =  W\left( \lambda^\beta(a\delta_s) \otimes 1 \right)(\delta_t \otimes v_{t^*}\xi) &= W(a\delta_{st} \otimes v_{t^*}\xi) \\
&= \delta_{st} \otimes \pi(a)v_{stt^*}\xi
    \end{align*}
\end{proof}


==> Random/Weak_amen.tex <==
\begin{remark}
Recall that by Example \ref{Oid2group} when $\G = \Gamma$ is a group, then the definition of $A(\G)$ reduces to the usual $A(\Gamma)$ defined for groups. From this, it follows that the same happens for weak amenability.    
\end{remark}
We now study how the Fourier algebra and weak amenability depend on the support of $\mu$. 
\begin{prop}
    Let $(\G,\mu)$ be a measured étale groupoid and $\Omega := \supp(\mu)$. Then there exists an inclusion $C_c(r^{-1}(\Omega)) \hookrightarrow A(\G) \subseteq L^\infty(\G)$.
\end{prop}
\begin{proof}
    Let $\varphi \in C_c(\G)$, it can be viewed as a section of the left regular Hilbert bundle $\Li^2(\G,\mu)$, simply by 
    $$
    \varphi(x)= \varphi|_{\G^x} \in \ell^2(\G^x), \quad \text{ for all } x \in \gob.
    $$
    Moreover, denoting by $\chi_X$ the unit section we get that for $\gamma \in G$,
    $$
(\overline{\varphi},\chi_X)_\lambda = \llangle \, \overline{\varphi}(r(\gamma)), L_\gamma( \chi_X(d(\gamma)) \, \rrangle_{\ell^2(\G^{r(\gamma)})} = \sum\limits_{\beta \in \G^{r(\gamma)}} \varphi(\beta) \chi_X(\gamma^{-1}\beta) = \varphi(\gamma).
    $$
    This defines a map $C_c(\G) \ni \varphi \rightarrow \varphi\in A(\G)$, which due to measure theoretic reasons may not be injective. However, will see that the restriction $C_c(r^{-1}(\Omega))  \rightarrow A(\G)$ will be. Indeed, let $\varphi,\psi \in C_c(\G)$ and 
    $$
    N := \{ \gamma \in \G: \varphi(\gamma) \neq \psi(\gamma) \} \subseteq r^{-1}(\Omega).
    $$
    Assume that $\varphi = \psi $ in $ A(\G) \subseteq L^\infty(\G)$, this means $\nu(N) = 0$. To prove thtat $\varphi = \psi$ in $C_c(r^{-1}(\Omega))$ we must show that $N = \emptyset$. Assume there exists a $\gamma \in N$, since $N$ is open and $\G$ is étale there exists an open bisection $U \subseteq N$ such that $\gamma \in U$. We have that
    $$
\mu(r(U)) = \nu(U) \leq \nu(N) = 0.
    $$
    On the other hand, $r(\gamma) \in r(U) \subseteq \Omega$ which means $\mu(r(U)) > 0$, a contradiction.
\end{proof}
Now, we prove that we can replace a net in $A(\G)$ with one in $C_c(r^{-1}(\Omega))$.
\begin{prop}
Let $(\G,\mu)$ be an étale measured groupoid and $\Omega := \supp(\mu)$. If $\G$ is weakly amenable, then there exists a net $(\varphi_i) \in C_c(\G)$ and a $C>0$ such that $\sup_i \|\varphi_i \|_{M_0A(\G)} \leq \cb(\G)$ and $\varphi_i \xrightarrow{} 1$ uniformly on compact sets. 
\end{prop}
\begin{proof}
    Let $(\psi_i) \in A(\G)$ be a net testifying the weak amenability of $\G$ and $C > 0$ such that $\sup_i \|\psi\|_{M_0A(\G)} \leq C$. Let $a \in C_c(\gob)$ be such that $a \geq 0$ and $a $
\end{proof}
We now prove that weak amenability only depends on the support of $\mu$.
\begin{prop}
Let $\G$ be an étale groupoid and $\mu_1,\mu_2$ be quasi-invariant probability measures on $\gob$. If $\supp(\mu_1) = \supp(\mu_2)$, then 
$$
\cb(\G,\mu_1) = \cb(\G,\mu_2).
$$
\end{prop}

==> Random/temp.tex <==
As it is the case with global actions, a partial action has an associated groupoid denoted by $X \rtimes G$, whose construction plays out very similarly. Its underlying set is 
$$
X \rtimes G := \{ (x,g): x \in D_g \} = \bigsqcup\limits_{g \in G} D_g \times \{g\},
$$
the source and range maps are $d(x,g) := (x,e)$ and $r(x,g) := (\alpha_t(x),e)$, respectively. Multiplication, when defined, is given by 
$$
(\alpha_t(x),g)(x,h) = (x,gh), \quad \text{ for all } g,h \in G \text{ and } x \in D_h.
$$


%%%%%%%%%%%%%%%%%%%%%%%%

Let us study the representation theory of $G$ that is adequate for our purpose.
\begin{defi}
    A map $u: G \rightarrow B(H)$ is said to a \textit{$*$-partial representation} of $G$ if for all $s,t \in G$, we have that 
    \begin{enumerate}[(i)]
        \item $u_1 = 1,$
        \item $u_su_tu_{t^{-1}} = u_{st}u_{t^{-1}}$,
        \item $u_{s^{-1}}u_su_t = u_{s^{-1}}u_{st}$,
        \item $u_{t^{-1}} = (u_t)^*$.
    \end{enumerate}
    If $u: G \rightarrow B(H)$ is a partial $*$-representation, $A$ is a $C^*$-algebra and $\pi: A \rightarrow B(H)$ is a $*$-homomorphism, the pair $(\pi,u)$ is said to be a \textit{covariant representation} of $(A,G,\beta)$ if for all $t \in G$ and $a \in E_{t^{-1}}$,
    $$
u_t \pi(a)u_{t^{-1}} = \pi(\beta_t (a)).
    $$
\end{defi}
We now proceed to build the left regular representation. We start with the space we are representing on, which counterintuitively will not be a Hilbert space but rather a Hilbert $C^*$-module over $A$. By \cite[Proposition 16.22]{exel2017partial} $A$

==> Universal_Groupoids/Intro.tex <==
\section{Weak Amenability of Universal Groupoids}

==> Universal_Groupoids/Restricted_Algebras.tex <==
\subsection{Restricted $C^*$-algebras of Inverse Semigroups}
In the previous section we constructed a groupoid $\G_u$ from an inverse semigroup $S$ that captured its representation theory. We now construct a new groupoid $\G_S$ from $S$, called the \textit{underlying groupoid} or \textit{Ehresmann groupoid} by introducing the restricted product for $s,t \in S$:
$$
s \cdot t = \begin{cases}
    st \quad &\text{ if } s^*s=tt^*, \\
    \text{undefined} &\text{ otherwise.}
\end{cases}
$$
Then $\G_S = (S,\cdot)$ is a discrete groupoid. In this section we will study representations of $S$ through $\G_S$. From this, we will define \textit{restricted representations} and build the \textit{restricted reduced $C^*$-algebra} of $S$. This theory was developed in \cite{amini2003restricted,amini2006restricted,amini2011restricted}. 
\begin{defi}
A map $\pi:S \rightarrow B(H)$ is said to be a \textit{restricted representation} if for all $s,t \in S$
$$ \pi(s)\pi(t) =
\begin{cases}
\pi(st) \quad &\text{ if } s^*s=tt^*, \\
    0 &\text{ otherwise.}
\end{cases}
$$
\end{defi}
Of course, there exists a \textit{restricted left regular representation} which is the map $\lambda^R: S \rightarrow B(\ell^2(S))$ defined for $s,t \in S$ by
$$
\lambda^R_s\delta_t =
\begin{cases}
\delta_{st} \quad &\text{ if } s^*s=tt^*, \\
    0 &\text{ otherwise.}
\end{cases} 
$$
The appropriate function algebra associated to restricted representations is still $\ell^1(S)$ (as a normed space) but the multiplication operation, which we abuse notation and also write it as $"\cdot"$ is different:
$$
f \cdot g(s) = \sum\limits_{s^*s=tt^*} f(st)g(s^*), \quad \text{ for all } f,g \in \ell^1(S) \text{ and } s \in S.
$$
To distinguish it, we will denote it by $\ell_R^1(H)$. The induced representation $\lambda^R: \ell^1_R(S) \rightarrow B(\ell^2(H))$ is faithful \cite[Lemma 4.1]{amini2003restricted} and we let the \textit{reduced restricted $C^*$-algebra} $C_R^*(S)$ be the completion of $\ell_R^1(H)$ under the norm $\|f\|_R := \|\lambda^R(f)\|$.

==> Universal_Groupoids/Universal_Groupoids.tex <==
\subsection{Universal Groupoids}
Let $X$ be a locally compact Hausdorff Space we denote by $\mathcal{I}(X)$ the set of all partial homeomorphisms of $X$, it is an inverse semigroup under the operation given by composition. In this section, we discuss actions of an inverse semigroup $S$ on a topological space $X$ and construct a groupoid associated to it. Following that we give the definition of an action of $S$ on a $C^*$-algebra $A$ and build the crossed product $A \rtimes S$.
\begin{defi}\label{actioninv}
An action of $S$ on $X$ is an inverse semigroup homomorphism $\alpha: S \rightarrow \mathcal{I}(X)$ such that
\begin{enumerate}[i]
    \item For every $s \in S$, $\alpha_s$ is continuous and has open domain on $X$;
    \item The union of the domains of all the $\theta_s$'s is $X$.
\end{enumerate}
\end{defi}
For each $s \in S$, we denote the domain of $\alpha_s$ by $D_s = D_{ss^*}$ and we define the subset of $X \times S$ 
$$
\Xi := \{(x,s) \in X \times S: x \in D_s \},
$$
on it we define an equivalence relation $(x,s) \sim (y,t)$ if and only if $x = y$ and there exists $e \in E$ such that $x \in D_e$ and $se = te$. For $(x,s) \in \Xi$ we denote its equivalence class by $[x,s]$ which is called the \textit{germ of $s$ at $x$}. We let $X \rtimes_\alpha S := \Xi / \sim$ (or just $X \rtimes S$ when $\alpha$ is obvious from the context) and define range and source maps as $d([x,s]) = [x,ss^*],r([x,s]) = [\alpha_s(x),ss^*]$, moreover we define a product by
$$
[\alpha_t(x),s][x,t] = [x,st]
$$
and inverse $[x,s]^{-1} = [\alpha_s(x),s^*]$. It remains to topologize $X \rtimes S$, for each $s \in S$ and open $U \subseteq D_s$, let 
$$
D(U,s) = \{ [x,s] \in X \rtimes S: x \in U \}
$$
\begin{prop}[{\cite[Proposition 4.17]{exel2008inverse}}]\label{gofgerms}
    The sets $D(U,s)$ are a basis for a topology on $X \rtimes_\alpha S$. Moreover, the operations defined above turn $X \rtimes_\alpha S$ into an étale groupoid.
\end{prop}
The groupoid $X \rtimes_\alpha S$ will be called the \textit{groupoid of germs of the action $(X,\alpha,S)$}.
\begin{example}\label{canact}
    Suppose $\G$ is any étale groupoid, recall the canonical action of $\G^{op}$ on $X = \gob$ given by
    $$
\alpha_U(x) = UxU^{-1}, \quad \text{ for all } x \in d(U),
$$
it is indeed an action in the sense of Definition \ref{actioninv}, with domain $d(U)$ and range $r(U)$. Moreover, if $S \subseteq \G^{op}$ is an inverse subsemigroup then one can restrict $\alpha$ to $S$ and the following proposition shows under what conditions we have $X \rtimes_{\alpha|_S} S \cong \G$.
\end{example}
\begin{prop}[{\cite[Proposition 5.4]{exel2008inverse}}]\label{isotrans}
Let $\G$ be an étale groupoid and $S \subseteq \G^{op}$ be an inverse subsemigroup such that 
\begin{enumerate}[(i)]
    \item $\bigcup\limits_{U \in S} U = \G$, and 
    \item for every $U,V \in S$ and $u \in U \cap V$, there exists $W \in S$ such that $u \in W \subseteq U \cap V$.
\end{enumerate}
Then we have that $X \rtimes_{\alpha|_S} S \cong \G$.
\end{prop}
\begin{defi}
    An inverse subsemigroup $S \subseteq \G^{op}$ is said to \textit{wide} if it satisfies the conditions of Proposition \ref{isotrans}.
\end{defi}
\begin{example}\label{universal groupoid}
    Let $S$ be an inverse semigroup (possibly with zero). We describe a way to construct from $S$ a groupoids of germs $\G_u$ called \textit{the universal groupoid} which was introduced in \cite{paterson2012groupoids} and we follow the notes \cite[Section 3.2]{anantharaman2016some}. Denote by $\widehat E$ the \textit{spectrum} of $S$, that is, the space of non-zero semigroup homomorphisms $\chi: E \rightarrow \{0,1\}$ such that $\chi(0) = 0$ (if $S$ has a zero) endowed with the topology of pointwise convergence. It is a locally compact totally disconnected space and if $S$ has a unit, $\widehat E$ is compact. \par
    The inverse semigroup $S$ acts on $\widehat E$ as follows. Let $s \in S$, we define $\alpha_s \in \mathcal{I}(\widehat E)$ with open domain $D_s = \{\chi \in \widehat E: \chi(s^*s) = 1 \}$ by 
    $$
\alpha_s(\chi)(e) = \chi(s^*es), \quad \text{for all } \chi \in \widehat E \text{ and } e \in E,
    $$
    it can be seen that $s \mapsto \alpha_s$ is an action of $S$ on $\widehat E$ and thus $\G_u := \widehat E \rtimes S$ is defined as the groupoid of germs associated with this action.
\end{example}
The relevant fact about the universal groupoid is that is captures the representation theory of $S$, indeed we have the isomorphisms $C^*(\G_u) \cong C^*(S)$ and $C_r^*(\G_u) \cong C_r^*(S)$ \cite[Theorems 4.4.1 and 4.4.2]{paterson2012groupoids}.
